Automatically Reconciling the Trade-off between Prediction Accuracy and Earliness in Prescriptive Business Process Monitoring

Prescriptive business process monitoring provides decision support to process managers on when and how to adapt an ongoing business process to prevent or mitigate an undesired process outcome. We focus on the problem of automatically reconciling the trade-off between prediction accuracy and prediction earliness in determining when to adapt. Adaptations should happen sufficiently early to provide enough lead time for the adaptation to become effective. However, earlier predictions are typically less accurate than later predictions. This means that acting on less accurate predictions may lead to unnecessary adaptations or missed adaptations. Different approaches were presented in the literature to reconcile the trade-off between prediction accuracy and earliness. So far, these approaches were compared with different baselines, and evaluated using different data sets or even confidential data sets. This limits the comparability and replicability of the approaches and makes it difficult to choose a concrete approach in practice. We perform a comparative evaluation of the main alternative approaches for reconciling the trade-off between prediction accuracy and earliness. Using four public real-world event log data sets and two types of prediction models, we assess and compare the cost savings of these approaches. The experimental results indicate which criteria affect the effectiveness of an approach and help us state initial recommendations for the selection of a concrete approach in practice.

==> abstract.tex <==
Prescriptive business process monitoring provides decision support to process managers on when and how to adapt an ongoing business process to prevent or mitigate an undesired process outcome.
We focus on the problem of automatically reconciling the trade-off between prediction accuracy and prediction earliness in determining when to adapt.
Adaptations should happen sufficiently early to provide enough lead time for the adaptation to become effective. 
However, earlier predictions are typically less accurate than later predictions.
This means that acting on less accurate predictions may lead to unnecessary adaptations or missed adaptations. 

Different approaches were presented in the literature to reconcile the trade-off between prediction accuracy and earliness. 
So far, these approaches were compared with different baselines, and evaluated using different data sets or even confidential data sets.
This limits the comparability and replicability of the approaches and makes it difficult to choose a concrete approach in practice. 

We perform a comparative evaluation of the main alternative approaches for reconciling the trade-off between prediction accuracy and earliness.
Using four public real-world event log data sets and two types of prediction models, we assess and compare the cost savings of these approaches.
The experimental results indicate which criteria affect the effectiveness of an approach and help us state initial recommendations for the selection of a concrete approach in practice.

\begin{keyword}
Predictive process monitoring \sep 
Prescriptive process monitoring \sep 
Process adaptation \sep
Machine learning \sep
Reinforcement learning \sep
Deep learning 

%% PACS codes here, in the form: \PACS code \sep code

%% MSC codes here, in the form: \MSC code \sep code
%% or \MSC[2008] code \sep code (2000 is the default)

\end{keyword}

%Proactive process adaptation can prevent and mitigate upcoming problems during process execution.
%Proactive adaptation decisions are based on predictions about how an ongoing process instance will unfold up to its completion.
%On the one hand, these predictions must have high accuracy, as, for instance, false negative predictions mean that necessary adaptations are missed.
%On the other hand, these predictions should be produced early during process execution, as this leaves more time for adaptations, which typically have non-negligible latencies.
%However, there is an important trade-off between prediction accuracy and earliness.
%Later predictions typically have a higher accuracy, because more information about the ongoing process instance is available.
%To make a trade-off between accuracy and earliness during predictive process monitoring, we use an ensemble of deep learning models.
%These ensembles can produce predictions at arbitrary points during process execution and in addition provide reliability estimates for each prediction, i.e., an indicator/probability of the prediction being correct.
%We use these reliability estimates to dynamically determine the earliest prediction with sufficient accuracy and use this prediction to trigger a proactive process adaptation.
%Experimental results indicate that our dynamic approach may offer cost savings of 27\% on average when compared to using a static prediction point for proactive process adaptation.



